Hypervolume-based column-and-constraint generation for bi-objective two-stage robust mixed-integer programs

Extending column-and-constraint generation (C&CG) for two-stage robust mixed-integer programs from the single-objective to the bi-objective setting is challenging: for a fixed first-stage decision and scenario, the second stage yields an entire nondominated set rather than a single objective value. We develop a C&CG algorithm that uses the hypervolume indicator - one of the most widely studied quality indicators in multi-objective optimization - to evaluate these sets and seeks a first-stage decision maximizing the worst-case hypervolume over a finite set of scenarios. To avoid the nonlinearities of an exact hypervolume formulation, we introduce a slab decomposition of the objective space that yields a linear mixed-integer master problem with an explicit bound on the discretization error. This bound enables a computable optimality-gap certificate and supports an adaptive algorithm that alternates between adding scenarios and refining the decomposition. We prove the correctness of the algorithm and establish sufficient conditions for its finite termination. Computational experiments on two-stage robust selection and assignment problems show that only a small number of scenarios need to be included in the master problem, even when the full scenario set contains 128 scenarios. Moreover, we identify the number of initial slabs as a key factor influencing the running time and develop a simple, instance-dependent rule for choosing the initial slab width that outperforms fixed choices on average for the selection problem and remains competitive for the assignment problem.

==> figures/grid-with-error-margin-code.tex <==
% h_i for each stripe from left to right
\def\heights{0, 0, 1, 2.3, 3.1, 3.1, 3.9, 3.9, 3.9, 5.2}
% x coordinate of the activating point for stripes from left to right. if 0 it is not shown
\def\pointsx{0,0,1.5,2.7,3.2,3.2,5.5,6.5,6.5,8.8}

% first convert list pointsx into indexed macros \PX1, \PX2, ...
\foreach[count=\i] \x in \pointsx {
	\expandafter\xdef\csname PX\i\endcsname{\x}
}
% convert heights[i] into H[i+1]
\foreach[count=\i] \h in \heights {
	\pgfmathtruncatemacro{\j}{\i+1} % j = i+1
	\expandafter\xdef\csname H\j\endcsname{\h}
}

% Draw grid
\draw[gray!50, line width=0.5pt] (0,0) grid[ystep=7] (10,7);

% areas
\foreach [count=\i] \h in \heights {
	% red area
	\fill[fillred, opacity=0.3] (\i-1,7-\h) rectangle ++(1,\h);
	
	% blue region
	\pgfmathsetmacro{\test}{\i>1 ? 1 : 0}
	\ifnum\test=1
	\fill[fillblue, opacity=0.3] (\i-2,7-\h) rectangle ++(1,\h-\csname H\i\endcsname);
	\fi
	
	% scatter activation points
	\pgfmathsetmacro{\test}{\h>0 ? 1 : 0}
	\ifnum\test=1
	\filldraw[pointred] (\csname PX\i\endcsname,7-\h) circle (2pt);
	\fi
}

% extra in right stripe
\node[pointred] at (9.3,1) {$\times$};
\fill[fillblue, opacity=0.3] (9,1) rectangle ++(1,7-\csname H11\endcsname - 1);


% Reference point (ref)
\filldraw[pointblue] (10,7) circle (2pt);

% axes
\draw[->, thick] (-0.7,0) -- (10.5,0);      % x-axis
\draw[->, thick] (-0.3,-0.5) -- (-0.3,7.5); % y-axis
\node[left] at (-0.7,0) {0};
\node[left] at (0,-0.8) {0};

% Annotations
\node[pointblue, right] at (10,7.2) {$\refpt$};

% Axes labels
\node at (-0.8,3.5) [rotate=90] {$f_2$};
\node at (5,-0.4) {$f_1$};




==> tables/sel-orientation.tex <==
\begin{table}
\centering\footnotesize\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|rrr|rrr||rrr|rrr}
\hline
 & \multicolumn{6}{c||}{horizontal slabs} & \multicolumn{6}{c}{vertical slabs} \\
 & \multicolumn{3}{c|}{$n=10$} & \multicolumn{3}{c||}{$n=20$} & \multicolumn{3}{c|}{$n=10$} & \multicolumn{3}{c}{$n=20$} \\
$p$ & 2 & 4 & 5 & 2 & 6 & 10 & 2 & 4 & 5 & 2 & 6 & 10 \\
\hline
Time [s] & 2.0 & 9.1 & 15.4 & 3.5 & 41.7 & 72.2 & 2.7 & 11.2 & 11.6 & 2.3 & 34.6 & 53.9 \\
Gap [\%] & 3.73 & 3.62 & 3.99 & 3.98 & 4.32 & 4.09 & 3.83 & 4.06 & 3.79 & 4.09 & 4.27 & 3.94 \\
$\min_{s} \HV^s(x^\ast)$ & 24.93 & 59.42 & 69.83 & 26.88 & 134.99 & 215.27 & 24.95 & 59.43 & 69.89 & 26.88 & 135.01 & 215.91 \\
Iterations & 7.3 & 6.5 & 6.6 & 6.6 & 7.3 & 6.7 & 6.9 & 6.7 & 6.3 & 5.6 & 6.9 & 5.8 \\
\hline
\end{tabular}
\caption{Horizontal versus vertical slab decomposition on the selection problem ($\TG=5\%$, $|S|=16$, starting slab width $w=40$, safety factor $\sigma=0.95$). Every column is one instance size $(n,p)$; each entry averages $10$ scenario seeds, and the two halves of the table are paired, i.e.\ they solve exactly the same $60$ instances. ``Time'' is the total wall-clock time, ``Gap'' the optimality gap certified on termination (target $5\%$), and $\min_{s\in S}\HV^s(x^\ast)$ the true worst-case hypervolume of the returned first-stage decision (in units of $10^3$). ``Iterations'' is the number of master solves.}
\label{tab:sel-orientation}
\end{table}

